Risk-Aware Real-Time Task Allocation for Stochastic Multi-Agent Systems under STL Specifications

This paper addresses the control synthesis of heterogeneous stochastic linear multi-agent systems with real-time allocation of signal temporal logic (STL) specifications. Based on previous work, we decompose specifications into sub-specifications on the individual agent level. To leverage the efficiency of task allocation, a heuristic filter evaluates potential task allocation based on STL robustness, and subsequently, an auctioning algorithm determines the definitive allocation of specifications. Finally, a control strategy is synthesized for each agent-specification pair using tube-based model predictive control (MPC), ensuring provable probabilistic satisfaction. We demonstrate the efficacy of the proposed methods using a multi-shuttle scenario that highlights a promising extension to automated driving applications like vehicle routing.

==> Graveyard.tex <==
 %%%%% Graveyard

% \section{introduction}

% Task assignment or allocation (TA) is a critical technology that ensures efficient and effective collaboration among multiple \uncertain{autonomous} agents~\cite{nunes2017taxonomy}. Given a group of agents and a list of tasks, TA decides which agent should take which task by searching for an optimal one-to-one matching~\cite{martello1987linear}. \uncertain{This renders a linear assignment problem that can be solved via linear programming~\cite{liu2015novel}.} An efficient type of TA approach is based on \textit{auction} algorithms that assign tasks according to the prices bid by the agents~\cite{bertsekas1992auction}. From a practical perspective, a price typically indicates the promised benefit when a certain task is assigned to an agent. In this sense, TA aims at maximizing the total prices for all assigned tasks or all agents. Decentralized auction algorithms have been proposed to leverage the computational efficiency by distributing the computational loads to individual agents \cite{zavlanos2008distributed, bai2022group}. Moreover, provably correct TA algorithms satisfying certain formal specifications have been developed with tasks formulated as linear temporal logic (LTL)~\cite{schillinger2018auctioning} or signal temporal logic (STL)\cite{leahy2021scalable} formulas. Beyond this, the efficiency of formal TA algorithms has been promoted with heuristic approaches, such as decision trees~\cite{li2023fast} and hierarchical models~\cite{schillinger2019hierarchical, luo2024simultaneous}.

%      In this paper, we consider task assignment to stochastic multi-agent systems with unbounded disturbance. The multi-agent system is assumed to be described by homogeneous agents with decoupled dynamics, and only through tasks can agents be connected. Each task will be described by signal temporal logic and is assumed to be unknown up to the time of assignment. Our objective is to determine an assignment and subsequently synthesise a controller for each agent, to ensure each task is fulfilled with a certain probability. To accomplish this objective, we consider the approach described in \ref{Fig:Approach1}. Here, we first determine a decomposition of the global specification into local specifications on a single-agent level, next heuristically filter the agent-specifications combinations, to afterwards compute for the remaining pairs an uncertainty value

%     However, agents with stochastic uncertainties no longer promise deterministic benefits in an auction due to the risk of failing the tasks within a certain time limit. Instead, each agent bid a probability price implying its anticipated ability to accomplish a task within the time limit~\cite{tihanyi2023multi}. Thus, \gls{ta} for uncertain agents renders a stochastic programming problem with probabilistic state-dependent constraints~\cite{gautier2023multi} and strict time constraints~\cite{wei2023towards}. A critical challenge of this problem is the dynamic adjustment of tasks according to the up-to-date status of agents~\cite{schillinger2018improving}. The dynamic adjustment should not only properly limit the computational complexities but also resolve the conflicts between the adjusted and the assigned tasks. When conflict resolution is infeasible, decomposition is needed to distribute a task to different agents~\cite{charitidou2021signal}. In~\cite{choudhury2022dynamic}, a dynamic \gls{ta} method has been developed for uncertain multi-agent systems with strict time constraints, where the conflicts between dynamically assigned tasks are resolved by minimizing the number of unsuccessful tasks. Simultaneous decomposition of tasks and agent groups has been efficiently realized in~\cite{leahy2022fast} based on modulo theories (SMT) and mixed-integer programming (MIP). Besides, the decomposition of formal task specifications has been studied in the temporal~\cite{zhang2023modularized} and the spatial dimensions~\cite{leahy2023rewrite}. In~\cite{galati2023auction}, human interventions are introduced to resolve conflicts by manually ordering task priorities. A survey on dynamic \gls{ta} of multi-agent systems can be referred to in~\cite{seenu2020review}.

%     Instead of dynamically adjusting predefined tasks, in this paper, we consider assigning sequential tasks that reflect the need of many practical scenarios, such as restaurant service robots that continually receive new guest orders. Not limited to the optimal \gls{ta} solution at a specific time, we argue that sequential \gls{ta} should instead ensure that all allocated tasks are accomplished above a predefined probability level, implying a limited task risk. This is more practical for sequentially assigned tasks considering that the real end users are typically concerned with an overall risk measure. 
%     Nevertheless, different from the existing dynamic \gls{ta} methods, agents should also proactively contribute to the risk limitation in sequential \gls{ta} by dynamically updating their behaviors. A similar argument has also been addressed in~\cite{fang2022automated} where deterministic agents proactively resolve the conflicts between the new and the existing tasks via a control strategy. Our previous work in~\cite{Enge2024} has also provided a risk-aware control rescheduling method for a single agent, which is promising to be extended to multi-agent systems. Based on the up-to-date behavior, each agent needs to dynamically adjust its probability price for sequential \gls{ta}, rendering a closed loop between agents and the \gls{ta} algorithm. {\color{red}Fig.1 or 2 could be moved to here.} Similar concepts addressing the interaction between the agents and the \gls{ta} algorithm have not been addressed in the literature.

%     In this paper, we propose a novel auction-based sequential \gls{ta} algorithm for multi-agent systems with stochastic uncertainties using the control rescheduling method proposed in~\cite{Enge2024}. Every time a new \gls{stl} task is given, it is first decomposed to \gls{stl} subformulas for individual agents to resolve potent conflicts. Then, an auction starts with each agent raising a probability price for each non-conflicting task to imply its likelihood of accomplishing the task, based on which a task scheduler solves an assignment plan. Each agent reschedules its control input to accomplish the assigned task by re-calculating the risk bounds using probabilistic reachable tubes. The complete process is illustrated in Fig.~\ref{}
% % {\color{red}We prove that the overall probability of accomplishing all assigned tasks is above a predefined probability level.} The remaining of the paper is organized as follows. ...

%     \paragraph{Literature review} The decomposition of a large multi-agent path planning problem under STL specifications is considered in \cite{Leahy2022}. Specifically, the authors present a computational framework for simultaneous decomposition and assignment, by splitting a multi-agent system and a global specification into subteams of agents and subformulas, respectively, the parallel execution of which ensures global satisfaction. The approach is based on satisfiability modulo theories (SMT) and mixed-integer programming (MIP). A rewrite method for jointly decomposing an STL formula and a team of agents is proposed in \cite{Leahy2023}. The approach relies on a set of formula transformations that facilitate decomposition. An algorithm for evaluating the transformation-based decomposition candidates is also provided. An optimization-based decomposition approach for splitting a fragment of STL into subformulas assigned to disjoint subsets of agents of a multi-agent team is proposed in \cite{Charitidou2022}. Therein, by parameterizing the underlying predicate functions by the infinity norm of agents' states, the volume of their superlevel set is maximized by solving a convex program over their parameters, the complexity of which depends on the multi-agent state dimension. An assume-guarantee framework for compositional control synthesis for an interconnected system under STL is presented in \cite{Liu2022}. This compositional framework enables the design of funnel-based feedback controllers under a decentralized architecture. A zonotope-based approach for state-space partitioning into finite cells is proposed in \cite{Ren2022}, which facilitates the decomposition of an STL specification into finite subformulas based on a reordering of the time constraints appearing in the STL specification.


 % \subsection{Tube-based MPC}

 %    In this section, we will define probabilistic reachable tubes, describe the tube-based MPC method to synthesizing and updating the controllers of individual agents and determine probabilistic guarantees for specification on sets of agents. \maico{This structure is of course still a work in progress and subject to changes.}

 %    \subsection{Optimization of the Assignment}

 %    Text

	% %%%%%%%%%%%%%%

	% \subsection{Probabilistic Reachable Tubes}

	% We define probabilistic reachable sets as follows, similar to \cite{Hewi2018}.
	% \begin{definition}[Probabilistic Reachable Sets] \label{Def:PRS}
	% 	A probabili-stic reachable set (PRS) of dynamic probability level $p$ for error dynamics \eqref{ErrorPart}, denoted by $\mathcal{R}^p$, is a set that satisfies
	% 	\begin{equation}\label{Eq:PRT}
	% 		e^i(0) = 0 \Rightarrow \Pr(e^i(k) \in \mathcal{R}^p) \geq p, \ \forall k \geq 0.
	% 	\end{equation}
	% \end{definition}
 %    \vspace{0.4em}
	% Definition \ref{Def:PRS} states that a PRS of probability level $p$ will contain at any time instance $k$ the accumulating error $e^i(k)$ with at least probability $p$, if the initial error satisfies $e^i(0)=0$. Moreover, due to the invariance property of PRS with respect to the accumulating error, a PRS may be defined at any time and can be moved over the time horizon without this influencing its probability level.

	% Multiple representations for probabilistic reachable sets exist, including the ellipsoidal representation. For simplicity, we will make the following assumption.

	% \begin{assumption} \label{Ass:Zero}
	% 	Distribution $\mathcal{Q}_w$ has zero mean.
	% \end{assumption}
 %    The above assumption is not necessary to obtain an ellipsoidal representation but will simplify most of the computations. The ellipsoidal representation is obtained from the multivariable Chebyshev inequality; details are given in \cite{Hewi2018}. Under Assumption \ref{Ass:Zero}, the ellipsoidal representation is given by
	% \begin{equation}\label{EllipNot}
	% 	\mathcal{R}^p= \{x \in \mathbb{R}^{n} \mid x^T \Sigma_{\infty}^{-1}x \leq \tilde p\},
	% \end{equation}
	% where $\Sigma_{\infty}$ solves the Lyapunov equation
	% \begin{equation} \label{Eq:Lyap}
	% 	A_K\Sigma_{\infty}A_K^T-\Sigma_{\infty}+\text{var}(\mathcal{Q}_w)=0,
	% \end{equation}
	% $p$ is the probability level, and
	% \begin{equation} \label{Eq:RelRadProb}
	% 	\tilde p=\frac{n}{1-p}.
	% \end{equation}
	% Since the variance of $\mathcal{Q}_w$ is assumed to be strictly positive definite and $A_K$ is stable, Lyapunov theory states that $\Sigma_{\infty}$ is strictly positive definite. Hence, in the sequel, we consider the transformed state and constraints for which $\Sigma_{\infty}=I_n$. We call these transformed dynamics \textit{the normalized dynamics}, and in the remainder, we maintain our notations as if the dynamics are normalized. Notice that each PRS is now a hypersphere with radius $\sqrt{\tilde p}$. Accordingly, Eq. \eqref{Eq:RelRadProb} is now a relation between the radius and the probability level of each PRS.

	% By defining a PRS $\mathcal{R}^{p_k}$ at each time instance $k \in \{0, \cdots, N\}$, we obtain a finite sequence of PRS called a probabilistic reachable tube $\mathcal{R}:=\{\mathcal{R}^{p_0}, \cdots, \mathcal{R}^{p_N}\}$. A probabilistic reachable tube can have either constant or varying diameter, with the former only if $p(i)=p(j)$ for all $i\leq j$. We define the risk level $r_k$ as an upper bound on the probability that $\mathcal{R}^{p_k}$ does not contain the error $e(k)$.

	% \begin{lemma}[Risk-Aware Tube Lemma \cite{Enge2024}] \label{Lem:Tube}
	% 	The risk that errors $\{e^i(0), \cdots, e^i(N)\}$ are not contained within a given probabilistic reachable tube $\{\mathcal{R}^{p_0}, \cdots, \mathcal{R}^{p_N}\}$ is at most
	% 	\begin{equation}
	% 		\bar r =\sum_{i = 1}^N (1-p_i).
	% 	\end{equation}
	% \end{lemma}

 %     \textbf{Approach 2: Generalized PRT.}
 %    Let $\phi$ be the non-decomposed specification assigned to agents $I=\{i_1,\cdots, i_m\}$. Given a sequence of tubes $\{\mathcal{R}^{i_1}, \cdots, \mathcal{R}^{i_m}\}$, one tube for each sub-specification $\phi_{i_j}$, we consider constructing a higher dimensional tube for which its projection on the state space of each agent $i_j$ will results in the projected tube being contained within tube $\mathcal{R}^{i_j}$. The result is a generalized tube which is contained within the constraints of the non-decomposed specification $\phi$ after which Lemma \ref{Lem:Tube} will give an upper bound on the risk of not satisfying specification $\phi$. \maico{Formal proof needs to be given, which depends on the decomposition framework.}
    
 %    The generalized PRT can be obtained by first computing at each time step $k$ over the set $i \in I$, the minimal probability level $\bar p_k$ over the set $\{\mathcal{R}^{p_k^i}| i \in I\}$ where $\mathcal{R}^{p_k^i}$ is the $k$-th element of $\mathcal{R}^i$, i.e, $\bar p_k \leq p_k^i$ for all $i \in I$. The new tube will be constructed by setting at time $k$ the radius of the generalized PRS equal to the corresponding radius of $\bar p_k$ which can be obtained from \eqref{Eq:RelRadProb} with $n$ equal to the dimension of agent $j$ given by $n_j$. The obtained radii on the generalized tube elements can similarly be translated towards probability levels using \eqref{Eq:RelRadProb} only now with $n$ equal to the higher dimension $\Sigma_{i \in I} n_i$. The result is a generalized tube $\{\mathcal{R}^{\bar p_0}, \cdots, \mathcal{R}^{\bar p_N}\}$.


    % \maico{The first approach would be to solve for each agent the tube-MPC completely independent. This can be achieved by providing each agent with a sub-specification and individual maximal risk. These individual maximal risks can be obtained from the maximal risk on the non-decomposed specification. This approach is useful as it allows us to directly use our previous work \cite{Enge2024} and Python code. Unfortunately, the results might be conservative.}
    
    % \maico{The second approach would consider a singular tube MPC optimization problem (different from Figure \ref{Fig:Approach1}) in which we combine the constraints of all agents together with constraints on the individual maximal risks of the sub-specifications, against the maximal risk of the non-decomposed specification. This approach \textbf{might!} be less conservative but will entail more computations and need us to rework the Python code. Additionally, we will have to spend a decent amount of space on introducing the new tube-MPC optimization problem. SINCE TIME IS LIMITED I OPTED FOR THE FIRST APPROACH WHEN WRITING THE APPROACH IN SECTION 2-D.}


    %%%% Case Study

    % We consider a multi-robot warehouse case handling scenario to validate the efficacy of the proposed method. The warehouse contains four charging stations `CH-X', with X\,$\in\!\{$A,B,C,D$\}$, four case shelves `CS-Z', with Z\,$\in\!\{$1,2,3,4$\}$, and one unloading point `ULP'. Four robots named A to D should fetch cases from the shelves and move those to the unloading point. The robots start from their respective charging stations and should return on request if possible. Meanwhile, all robots are restricted within the warehouse denoted by `BOX' and should avoid collision with two obstacles, `OB-Y', with Y\,$\in\!\{$1,\,2$\}$. Based on these essential descriptions, this case study is concerned with dynamically assigned specifications, i.e., new task specifications (either global or local ones) may be assigned at any time $k \in \{0,1,\cdots,N\!-\!1\}$. The specifications are defined as follows, where we consider a finite control horizon $N\!=\!25$ and use $\mu_{\mathrm{R}}\!:=\!x_k \!\in\!\mathrm{R}$ to denote a predicate that the state $x_k$ of a robot $X$ is within a region $\mathrm{R}$ for any time $k\in[0,N]$.

    %The motion planning scenario is illustrated in Fig.~\ref{Fig:StateMeas} which contains a safety set $S:=\{(x_1, x_2) \in \mathbb{R}^2 \mid -10 \leq x_1 \leq 10 \text{ and } -2 \leq x_2 \leq 10\}$, a home set $H:=\{(x_1, x_2) \in \mathbb{R}^2 \mid -10 \leq x_1 \leq 10 \text{ and } -2 \leq x_2 \leq 0\}$, an obstacle $O:=\{(x_1, x_2) \in \mathbb{R}^2 \mid -2 \leq x_1 \leq 2 \text{ and } 3 \leq x_2 \leq 10\}$, two targets $T_1:=\{(x_1, x_2) \in \mathbb{R}^2 \mid -10 \leq x_1 \leq -8 \text{ and } 8 \leq x_2 \leq 10\}$ and $T_2:=\{(x_1, x_2) \in \mathbb{R}^2 \mid 7 \leq x_1 \leq 9 \text{ and } 7 \leq x_2 \leq 9\}$, and a charger $C:=\{(x_1, x_2) \in \mathbb{R}^2 \mid -8 \leq x_1 \leq -3 \text{ and } 2 \leq x_2 \leq 4\}$. 

    % This case study considers a reach-avoid problem in which new reach objectives are dynamically assigned. More precisely, the specifications $\{\phi_0, \phi_1, \phi_2, \phi_3\}$ are assigned to the robot at times $k=0, \ k=5, \ k=15$ and $k=20$, respectively. Here $\phi_0:=\square_{[0,40]}\left[(x(k) \in S) \wedge \lnot (x(k) \in O)\right]$, $\phi_1:=\lozenge_{[20,30]}\left[(x(k) \in T_1) \vee (x(k) \in T_2)\right]$, $\phi_2:=\lozenge_{[20,25]}(x(k) \in C)$, and $\phi_3:=\lozenge_{[25, 30]}\square_{[0,5]}(x(k) \in H)$. Additionally, we specify that the control inputs are limited by $-2 \leq u(k) \leq 2$ for all $k \in \{0,1,\cdots, N-1\}$. We use the \textit{stlpy} toolbox to synthesize our controller~\cite{Kurt2022}. The results are shown in Fig. \ref{Fig:StateMeas} and Table \ref{tab:SpecLowBound}.
	
	% \begin{table}[htp]
	% 	\centering
	% 	\resizebox{0.6\columnwidth}{!}{%
	% 		\begin{tabular}{|l|c|c|c|c|}
	% 			\hline
	% 			& \multicolumn{1}{l|}{$\phi_0$} & \multicolumn{1}{l|}{$\phi_1$} & \multicolumn{1}{l|}{$\phi_2$} & \multicolumn{1}{l|}{$\phi_3$} \\ \hline
	% 			$k=k_i$ & 0.40                           & 0.10                           & 0.05                          & 0.10                           \\ \hline
	% 			$k=N$  & 0.40                           & 0.10                           & 0.05                          & 0.10                           \\ \hline
	% 		\end{tabular}%
	% 	}
	% 	\vspace{1em}
	% 	\caption{\small A table containing the upper bound risks of $\phi_i$ at time of acceptance $k_i$ and after runtime.}
	% 	\label{tab:SpecLowBound}
	% \end{table}

    % From Fig. \ref{Fig:StateMeas}, we notice that at time $k=5$, the robot was scheduled to move towards the right target, only for it to move to the left target when it was additionally tasked with recharging its battery at time $k=15$. This result clearly illustrates that our control scheme allows the robot to make changes during runtime to accomplish as many tasks as possible. Additionally, upper bound risks on specifications, see Table \ref{tab:SpecLowBound}, remained below the maximum of $r_{\pi,\max}=0.5$. This result illustrates the ability to obtain valid probabilistic guarantees. Finally, it can be seen that state updates likely influence the robot's movement since the blue trajectory clearly differs from the green trajectory around the charger, something which is unlikely to be attributed only to the additive disturbances due to the variance being relatively small.



        % Let $\phi$ be the non-decomposed specification. Given a sequence of sub-specifications $\{\phi_1, \cdots, \phi_{\nu}\}$ with individual maximal risks $\{r_{\phi_1, \max}, \cdots, r_{\phi_{\nu}, \max}\}$, the union bound argument, denoted by
    % \begin{equation} \label{Eq:UnionBound}
    %     \mathbb{P}(\bigcup_{i=1}^N A_i) \leq \sum_{i=1}^N \mathbb{P}(A_i),
    % \end{equation}
    % allows us to compute an upper bound on the risk of not satisfying $\phi$. This is given by
    % \begin{equation} \label{Eq:UppRisk}
    %     r=\sum_{i=1}^{\nu} r_{\phi_i, \max}.
    % \end{equation}
    % Relation \eqref{Eq:UppRisk} allows us to assign to each sub-specification $\phi_i$ a maximal risk $r_{\phi_i,\max}$ to ensure specification $\phi$ has at most risk $r_{\phi,\max}$. Amongst many options, the most simplistic would be to take the average, i.e., 
    % \begin{equation} \label{Eq:RiskAve}
    %     r_{\phi_i,\max} = \frac{r_{\phi,\max}}{\nu}.
    % \end{equation}


    %Consider the collision avoidance formula $\phi=\square_{[a,b]}\neg\mu$, where $\mu:=(h(x)\geq 0)$, with $h(x)={\tiny\begin{bmatrix}
    %     \bm{I}\\-\bm{I}
    % \end{bmatrix}x-\bm{1}_4}$, $\bm{1}_4=[1,1,1,1]^T$, and $x=[x_1\ x_2]^\intercal$, $x_i\in\mathbb{R}$ being the state of agent $i=1,2$. Let $H=\{x \mid h(x)\geq0\}$, with $\mathbb{B}_{\mathrm{out}}(H)\equiv H$. Then, we have that $\dec(\neg\mu,2)=\neg \mu_1 \wedge \neg \mu_2$, where $\mu_1:=(-1 \leq x_1 \leq 1)$ and $\mu_2:=(-1\leq x_2 \leq 1)$, is a valid decomposition. Finally, $\dec(\phi,2)=\wedge_{i=1}^2 \square_{[a,b]}\neg \mu_i$. 


    %{\color{red}Existing work on control synthesis with STL specification includes, amongst others, , which considers (tube-based) model predictive control (MPC) for single-agent stochastic systems; \cite{Liu2017,fang2022automated} which considers multi-agent deterministic systems; and  which consider respectively uncertain and stochastic multi-agent systems. However, none consider real-time assignments of tasks for stochastic multi-agent systems.}({\color{green}We need to further specify this part, probably following the way in ADHS paper.})
